Verification and Validation Issues in Systems of Systems

The cutting edge in systems development today is in the area of "systems of systems" (SoS) large networks of inter-related systems that are developed and managed separately, but that also perform collective activities. Such large systems typically involve constituent systems operating with different life cycles, often with uncoordinated evolution. The result is an ever-changing SoS in which adaptation and evolution replace the older engineering paradigm of "development". This short paper presents key thoughts about verification and validation in this environment. Classic verification and validation methods rely on having (a) a basis of proof, in requirements and in operational scenarios, and (b) a known system configuration to be proven. However, with constant SoS evolution, management of both requirements and system configurations are problematic. Often, it is impossible to maintain a valid set of requirements for the SoS due to the ongoing changes in the constituent systems. Frequently, it is even difficult to maintain a vision of the SoS operational use as users find new ways to adapt the SoS. These features of the SoS result in significant challenges for system proof. In addition to discussing the issues, the paper also indicates some of the solutions that are currently used to prove the SoS.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{Larsen, Legay, Nyman (Eds.): 1st Workshop on \\
Advances in Systems of Systems (AiSoS 2013)\\
EPTCS 133, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.133.1}{10.4204/EPTCS.133.1}}

